Probabilistic Causal Analysis of Social Influence

Mastering the dynamics of social influence requires separating, in a database of information propagation traces, the genuine causal processes from temporal correlation, i.e., homophily and other spurious causes. However, most studies to characterize social influence, and, in general, most data-science analyses focus on correlations, statistical independence, or conditional independence. Only recently, there has been a resurgence of interest in "causal data science", e.g., grounded on causality theories. In this paper we adopt a principled causal approach to the analysis of social influence from information-propagation data, rooted in the theory of probabilistic causation. Our approach consists of two phases. In the first one, in order to avoid the pitfalls of misinterpreting causation when the data spans a mixture of several subtypes ("Simpson's paradox"), we partition the set of propagation traces into groups, in such a way that each group is as less contradictory as possible in terms of the hierarchical structure of information propagation. To achieve this goal, we borrow the notion of "agony" and define the Agony-bounded Partitioning problem, which we prove being hard, and for which we develop two efficient algorithms with approximation guarantees. In the second phase, for each group from the first phase, we apply a constrained MLE approach to ultimately learn a minimal causal topology. Experiments on synthetic data show that our method is able to retrieve the genuine causal arcs w.r.t. a ground-truth generative model. Experiments on real data show that, by focusing only on the extracted causal structures instead of the whole social graph, the effectiveness of predicting influence spread is significantly improved.

==> experiments.tex <==
%!TEX root = cikm18.tex

%We measured the performance of our approach on both simulated data, where the true model generating the data is given, as well as on real data. The first set of tests allowed us to ensure the validity of our approach and the correctness of its implementation. With the second set of tests, instead, we proved the practical relevance of our approach on real-world datasets.

%\subsection{Experiments on synthetic data} \label{sec:synthetic_data}
\spara{Synthetic data.}
We generated synthetic data as follows.
\begin{enumerate}
\item Randomly generate a directed graph $G = (V,A)$ (our social graph) with $n$ nodes and density $\delta_G$.
% density representing the social network $G$. In this step, we start from the empty graph and add arcs to the network by randomly selecting them with uniform probability until we reach the desired density.
\item Randomly partition the nodes of the generated graph $G$ into a set of $k$ groups $P = \{S_1,\ldots,S_k\}$, with $\cup_{i=1}^k S_i = V$ such that: $(i)$ $\forall i \in [1,k]$, $G(S_i)$ is weakly-connected, $(ii)$ the cardinality of each group is bounded by $[\mbox{card}_{min},\mbox{card}_{max}] \in (0,n)$ and $(iii)$ the number of overlapping nodes between any pair of groups is bounded by $\mbox{card}_{overlap} \leq \mbox{card}_{max}$.
\item Generate a causal \DAG\ $G_{cause_i}$ of density $\delta_{G_{cause}}$ for each of the $k$ groups. Namely, we obtain $\mathbb{G}_{cause} = \{G_{cause_1},\ldots,G_{cause_k}\}$, by considering the union graph of each partition independently and then randomly removing arcs from it in order to discard cycles. Then, we assign to each remaining edge a random value bounded by $[p_{min},p_{max}] \in (0,1)$, representing the conditional probability of the child node given the connected parent. Notice that in these settings, we assume the probability of any child given the absence of all its parents to be $0$.
\item Generate a set of $o_k$ observations for each of the $k$ groups in terms of triples $\langle v, \phi, t \rangle$ (i.e., the database of propagation traces $\D$) such that each user performs at least one action, but, at the same time, she does not perform an action on at least one item of each cluster. To do this, we sample a set of traces with probability distributions induced by the causal \DAGs; in this way, we obtain a set of users\/entities that are observed in the trace. We then add the time $t$ to each observation randomly, but still consistently with the total ordering defined by the \DAG.
\end{enumerate}

Moreover, we model noise in the data by considering probabilities $e_+, e_- \in (0,1)$, representing false-positive and false-negative observations in each item, respectively, i.e., the probability of adding or removing from $\D$ a certain triple $\langle v, \phi, t \rangle$, independently of how it was sampled from the underlying causal process.
Notice that these two sources of noise aim at modeling imperfect regularities in the causal phenomena in terms of either false positive/negative observations or noise in the orderings among the events.

We use the following metrics of performance assessment:
\begin{itemize}
\item {\em Partitioning:} the objective here is estimating how well our partitioning step can effectively group users involved in the same causal process. To this extent, we consider the clusters of users belonging to the same \DAGs\ and we adopt the well-established Normalized Mutual Information (NMI) measure \cite{danon2005comparing}) to measure the similarity between the clusters identified by our method and the ground-truth clusters.
%, suitably adjusting the metric for our fuzzy clusters. If one element is in more than one cluster, we assign randomly one out of many (to make the cluster hard and no longer fuzzy/soft). Then repeat this assessment $100$ times (with different random assignments of clustering). For each iteration, compute the normalized mutual information (value in $0,1$) between the ground truth and the inferred model. We consider as a final metric the median of the results at each iteration.
\item {\em Causal topology:} we also assess by Hamming distance how the causal structure inferred by step 2 of our approach reflects the generative model \cite{hamming1950error}, i.e., by counting the minimum number of substitutions required to remove from the imputed topologies any inconsistency when compared with the generative ones. Specifically, we first build the union graph of the causal \DAGs of each cluster to obtain the graph of all the true causal claims. We do this for both the generative \DAGs and the inferred ones. Then, we compute the Hamming Distance from the ground truth and the inferred structures as a metric for the performance. Namely, we evaluate our performance in terms of $accuracy = \frac{(TP + TN)}{(TP + TN + FP + FN)}$, with $TP$ and $FP$ being the true and false positive and $TN$ and $FN$ being the true and false negative\footnote{We define positive (resp. negative) an arc that is present (resp. absent) in the network.} between the simulated topologies and the reconstructed ones.
\end{itemize}



% The pseudocode for the data generation is shown in Algorithm \ref{alg:data_no_noise}. The generation of the causal structures $\mathbb{G}_{cause}$ and of the database of the noise free propagation traces $\D_{nf}$ consists of $4$ steps.

% Subsequently, the types of noise defined above are added to these noise free propagation traces $\D_{nf}$ to generate the actual database of the propagation traces $\D$.

% \begin{algorithm}
% \caption{Noise Free Data Generation}
% \label{alg:data_no_noise}
% \begin{algorithmic}[Noise Free Data Generation]
% \STATE{\textbf{STEP 1: Structure of the Social Network $G$}}
% \STATE{$n$, number of nodes in the social network.}
% \STATE{$\delta_G$, density of the social network.}
% \STATE{Generate a random graph of $n$ nodes and $\delta_G$ density representing the social network.}
% \RETURN $G$, the social network.
% \STATE{\textbf{STEP 2: Partitioning $G$ into $k$ clusters $P$}}
% \STATE{$card_{min}$, minimum cardinality of each cluster.}
% \STATE{$card_{max}$, maximum cardinality of each cluster.}
% \STATE{$card_{overlap}$, maximum number of overlapping nodes.}
% \STATE{Partition the nodes of the graph in $k$ groups with overlap $card_{overlap}$ and cardinality uniformly sampled in $[card_{min},card_{max}]$.}
% \RETURN $P$, the partitions.
% \STATE{\textbf{STEP 3: Generate the set of causal \DAGs\ $\mathbb{G}_{cause}$}}
% \STATE{$\delta_{cause}$, density of the causal graphs.}
% \STATE{Randomly choose a set of arcs of the social network to generate a weakly connected \DAGs\ .}
% \STATE{Randomly sample a probability values in $(0,1)$ for each arc.}
% \RETURN $\mathbb{G}_{cause}$, the causal \DAGs\ .
% \STATE{\textbf{STEP 4: Sampling of $o$ observations per cluster}}
% \STATE{$o$, number of triples $\langle v, \phi, t \rangle$ to be sampled.}
% \STATE{Sample from the \DAGs\ and generate a random total order for the traces consistend with the poset induced by the \DAGs\ .}
% \RETURN $\D_{nf}$.
% \end{algorithmic}
% \end{algorithm}


\begin{figure}[t!]
\centering
\vspace{-4mm}
\includegraphics[width=.34\textwidth]{fig/simulations_execution_time}
\vspace{-6mm}
\captionsetup{justification=justified,singlelinecheck=off,font={stretch=0.7}}
\caption{\footnotesize Execution time on synthetic data. We considered $8$ configurations defines by coombinations of $\alpha \in [0.1, 0.25]$ and $\eta \in [0, 1, 3, 5]$. Each bar report the execution time for each configuration.} \label{fig:time_simulations}
\end{figure}

We generated synthetic data for $100$ independent runs. In each run we considered social graphs of $n=100$ nodes of density uniformly sampled in $\delta_G = [5\%,10\%]$. Moreover, we partitioned each randomly generated social network in $k=10$ clusters of $\mbox{card}_{min} = 8$, $\mbox{card}_{max} = 12$ and $\mbox{card}_{overlap} = 10$ nodes ($1\%$). Given each cluster, we generated causal \DAGs\ of $\delta_{G_{cause}} = [35\%,50\%]$ and $[p_{min},p_{max}]$ uniformly sampled in $(0,1)$. For our noise-free model, we constrain the process of social influence, by assuming a perfect regularity in the action of directly connected users: all the actions of a child user follow those of one of its parents, thus letting us  constrain the induced distribution of the generating \DAG as follows: with $u$ being a user in the network and $P(u)$ all the users with arcs pointing to $u$ ($u$'s parent set), the probability of observing any action from $u$ is $0$ if none of $u$'s parents had performed an action before (i.e., $P(u)$ are independently influencing $u$).

Given these settings, we sampled databases of propagation traces $\D$ at different sample sizes, i.e., we considered sample sizes of $500$, $1000$ and $5000$ traces. The traces were sampled across the $k=10$ groups to guarantee a sample size for each of them with the mean $+/-$ $[0\%,50\%]$, e.g. for size $500$ traces to each cluster are assigned between $25$ and $75$ samples.
%
Finally, we generated noisy datasets with a probability of generating a noisy entry of $[5\%,10\%]$ per entry. Any noisy entry had uniform probability of being either a false positive/negative. % or a swap.
We experimented with a total of $9$ ($3$ sample levels and $3$ noise levels) different settings.

On the simulations as described above, we tested our two-step methodology setting $K=100$, and considering different values of $\alpha \in [0.1, 0.25]$ and $\eta \in [0, 1, 3, 5]$
%, leading to a final list of $72$ possible configurations.
%
First, we evaluated the execution time of our clustering method for all the  configurations (Figure \ref{fig:time_simulations}). The figure shows the execution time for the $8$ configurations of $\alpha$ and $\eta$ just described. As depicted in the figure, the different values of $\alpha$ and $\eta$ do not seem to have a significant impact to the execution time.
%
Then we evaluated the performance of both the clustering (Figure \ref{fig:nmi_clustering_simulations_100_sampling} shows the results for the case of $\alpha = 0.1$ and $\eta = 0$), and of the final causal graphs obtained using BIC as a regularizator (Figure \ref{fig:accuracy_inference_bic_simulations_100_sampling} shows the results for BIC with the same configurations as before). The maximum likelihood fit was performed on the binarized version of the synthetic data, using 0 to model absence of an action and 1 to represent the fact that the given user performed it.
%
Overall, the performance metrics for both the clustering and of the inferred causal networks are similar across all the configurations, although, as expected, they progressively degrade as the applied noise increases. The values of normalized mutual information are consistently above $0.65$, while the accuracy in the inferred causal structures is above $0.90$ in almost all the settings of noise and sample size.

% \begin{figure}[t!]
% \centering
% \includegraphics[width=.40\textwidth]{fig/nmi_clustering_simulations_comparison_sampling}\\
% \caption{\small \emph{Normalized Mutual Information across all configurations. We considered $8$ configurations for the $\alpha \in [0.1, 0.25]$ and $threshold_{agony} \in [0, 1, 3, 5]$ parameters, plus $3$ sample sizes ($500$, $1000$ and $5000$ trances) and $3$ noise levels ($0\%$, $5\%$ and $10\%$) for the simulations for a total of $72$ configurations.}} \label{fig:nmi_clustering_simulations_comparison_sampling}
% \end{figure}

\begin{figure}[!t]
\centering
\vspace{-4mm}
\includegraphics[width=.34\textwidth]{fig/nmi_clustering_simulations_100_sampling}
\vspace{-4mm}
\captionsetup{justification=justified,singlelinecheck=off,font={stretch=0.7}}
\caption{\footnotesize NMI of the clusters identified by the proposed method vs. ground-truth clusters, for $\alpha = 0.1$ and $\eta = 0$. For each setting, sample sizes of $500$, $1000$, $5000$ traces, and noise of $0\%$, $5\%$, $10\%$ are considered.}
\label{fig:nmi_clustering_simulations_100_sampling}
\end{figure}

\begin{table*}[!t]
\centering
\vspace{-4mm}
\footnotesize
\captionsetup{justification=justified,singlelinecheck=off,font={stretch=0.7}}
\caption{{ \footnotesize Characteristics of the datasets used in the experiments: number of observations ($|\A|$); number of propagations/\DAGs\ ($|\D|$); nodes ($|V|$) and arcs ($|A|$) in the input graph $G$; min, max, and avg number of nodes in a \DAG\ in $\D$ ($n_{min}$, $n_{max}$, $n_{avg}$);  min, max, and avg number of arcs in a \DAG\ in $\D$ ($m_{min}$, $m_{max}$, $m_{avg}$).}\vspace{-3mm}}
%\begin{tabular}{@{}c@{}@{ \ }|r@{}@{ \ }r@{}@{ \ }r@{}@{ \ }r@{}@{ \ }|r@{}@{ \ }r@{}@{ \ }r@{}@{ \ }r@{}@{ \ }r@{}@{ \ }r@{}}
\begin{tabular}{c|rrrr|rrrrrr}
\hline
 & $|\A|$ & $|\D|$ & $|V|$ & $|A|$ & $n_{min}$ & $n_{max}$ & $n_{avg}$  & $m_{min}$ & $m_{max}$  & $m_{avg}$\\
\hline
%\flixster  &  6\,529\,012  &  11\,659  &  29\,357  &  425\,228  & 14 &  16\,129  & 561 & 13 &  85\,165  &  1\,561 \\
\lastfm  &  1\,208\,640  &  51\,495  &   1\,372 &  14\,708 & 6 & 472 & 24 & 5 &  2\,704 & 39\\
\twitter  &  580\,141  &  8\,888  &  28\,185  &  1\,636\,451  & 12 &  13\,547  & 66 & 11 &  240\,153  & 347\\
%\flickr  & 2\,026\,062 & 45\,124 & 441\,052 & 1\,739\,842 & 30 & 196 & 43 & 30 & 196 & 44 \\
% \wikipedia  & 50\,092 & 5\,477 & 39\,756 & 46\,610 & 4 & 125 & 9 & 4 & 131 & 9 \\
\hline
\end{tabular}
\vspace{-2mm}
\label{tab:dataset}
\end{table*}


% \begin{figure}[t!]
% \centering
% \includegraphics[width=.40\textwidth]{fig/accuracy_inference_aic_simulations_comparison_sampling}\\
% \caption{\small \emph{Accuracy for AIC across all configurations. We considered $8$ configurations for the $\alpha \in [0.1, 0.25]$ and $threshold_{agony} \in [0, 1, 3, 5]$ parameters, plus $3$ sample sizes ($500$, $1000$ and $5000$ trances) and $3$ noise levels ($0\%$, $5\%$ and $10\%$) for the simulations for a total of $72$ configurations.}} \label{fig:accuracy_inference_aic_simulations_comparison_sampling}
% \end{figure}

% \begin{figure}[!t]
% \centering
% \includegraphics[width=.40\textwidth]{fig/accuracy_inference_aic_simulations_500_sampling}\\
% \caption{\small \emph{Accuracy for AIC for the case of $50$, $100$ and $500$ sampling iterations, with $\alpha = 0.1$ and $threshold_{agony} = 0$. For each setting, $3$ configurations of sample size ($500$, $1000$ and $5000$ trances) and $3$ noise levels ($0\%$, $5\%$ and $10\%$) are considered.}} \label{fig:accuracy_inference_aic_simulations_500_sampling}
% \end{figure}

% \begin{figure}[t!]
% \centering
% \includegraphics[width=.40\textwidth]{fig/accuracy_inference_bic_simulations_comparison_sampling}\\
% \caption{\small \emph{Accuracy for BIC across all configurations. We considered $8$ configurations for the $\alpha \in [0.1, 0.25]$ and $threshold_{agony} \in [0, 1, 3, 5]$ parameters, plus $3$ sample sizes ($500$, $1000$ and $5000$ trances) and $3$ noise levels ($0\%$, $5\%$ and $10\%$) for the simulations for a total of $72$ configurations.}} \label{fig:accuracy_inference_bic_simulations_comparison_sampling}
% \end{figure}








\spara{Real data.}
We also experimented with $2$ real-world datasets, whose main characteristics are summarized in Table \ref{tab:dataset}. %Flixster \cite{flixster_bib}, Last.fm \cite{last.fm_bib}, Twitter \cite{twitter_bib} and Wikipedia \cite{wikipedia_bib}.

%\flixster\ (\texttt{www.flixster.com}).
%Flixster is a social movie site where people can meet each other based on tastes in movies. The graph $G$ corresponds to the social network underlying the site. The entities in $\E$ are movies, and an observation $\langle u, \phi, t\rangle$ is included in $\A$ when the user $u$ rates for the first time the movie $\phi$ with the rating happening at time $t$.
%
%\smallskip

\lastfm\ (\texttt{www.last.fm}).
Lastfm is a music website, where users listen to their favorite tracks and communicate with each other. The dataset was created starting from the \textit{HetRec 2011 Workshop} dataset available at \url{www.grouplens.org/node/462}, and enriching it by crawling. The graph $G$ corresponds to the friendship network of the service. The entities in $\E$ are the songs listened to by the users. An observation $\langle u,\phi, t \rangle \in \A$ means that the first time that the user $u$ listens to the song $\phi$ occurs at time $t$.

\twitter\ (\texttt{twitter.com}).
We obtained the dataset by crawling the public timeline of the popular online microblogging service.
The nodes of the graph $G$ are the Twitter users, while each arc $(u,v)$ expresses the fact that $v$ is a follower of $u$. The entities in $\E$ correspond to URLs, while an observation $\langle u,\phi, t \rangle \in \A$ means that the user $u$  (re-)tweets (for the first time) the URL $\phi$ at time $t$.

%\smallskip
%
%\wikipedia\ (\texttt{www.wikipedia.com}).
%We created this dataset by looking at the browsing sessions of the popular online encyclopedia. Any node of the graph $G$ corresponds to a Wikipedia page, while an arc $(u,v)$ is present in $G$ if there exists a browsing session where the page $v$ has been reached from the page $u$, even making use of intermediate pages external to the website.
%%a hyperlink exists from  a page in the photostream $u$ to a page in the photostream $v$.
%An entity $\phi \in \E$ corresponds to a browsing session. An observation $\langle u, \phi, t \rangle \in \A$ means that the page $u$ is visited during the session $\phi$ at time $t$. For each page, we consider only the first visit among the multiple ones possibly performed within the same session.


On such datasets, we run the proposed algorithm setting $\alpha = 0.20$, $\eta = 5$, and $K = 500$. %We report in Figure \ref{fig:time_real_data} the execution time for all the datasets for the case of $100$ sampling iterations.
As for before, the maximum likelihood fit was performed on the binarized version of the datasets, using 0 to model absence of an action and 1 to represent the fact that the given user performed it. Both AIC and BIC were used as regularized likelihood scores.
%The execution time is obviously proportional to the size of the underlying social network, with Wikipedia being the smallest leading to runs in the order of minutes. The most challenging dataset is Flixster.

\begin{figure}[t]
\centering
\vspace{-4mm}
\includegraphics[width=.34\textwidth]{fig/accuracy_inference_bic_simulations_100_sampling}
\vspace{-4mm}
\captionsetup{justification=justified,singlelinecheck=off,font={stretch=0.7}}
\caption{\footnotesize Accuracy of the proposed method, for BIC regularizator, $\alpha = 0.1$, $\eta = 0$. For each setting, sample sizes of $500$, $1000$, $5000$ traces, and noise of $0\%$, $5\%$, $10\%$ are considered.} \label{fig:accuracy_inference_bic_simulations_100_sampling}
\end{figure}

% \begin{figure}[!t]
% \centering
% \includegraphics[width=.40\textwidth]{fig/real_data_execution_time}\\
% \caption{\small \emph{Execution time on real data. We considered $4$ datasets, Flixster \cite{flixster_bib}, Lastfm \cite{last.fm_bib}, Twitter \cite{twitter_bib} and Wikipedia \cite{wikipedia_bib} and we report in the Figure the execution time of our clustering algorithm with a total of $100$ sampling iterations.}} \label{fig:time_real_data}
% \end{figure}


Here no ground truth is available.
Thus, we used the well-established spread-prediction task as a proxy to evaluate our approach. This task aims at predicting the expected number of nodes that eventually get activated given a propagation model \cite{goyal2011data}. We considered the propagation model of \cite{barbieri2013cascade} and ran the method with a total of $10,000$ Monte Carlo simulations as suggested in \cite{barbieri2013cascade}.
%However, this procedure is computational intensive and, because of this, we were precluded to consider the largest datasets and, for computational reasons, we evaluated spread-prediction only for Lastfm and Twitter. For these two datasets,
We applied the method in \cite{barbieri2013cascade} to different inputs: first we considered the original social network and we used it as a baseline to evaluate our performance; then we considered the causal arcs inferred by our approach with both AIC and BIC regularizations. For each inputs, we also attached weights to each arc connecting a node $u$ to its child $v$ as the conditional probability of an action of the child to be observed when an action of the parent was performed before.

We show the mean squared error between the test set and the predicted traces for \lastfm\ and \twitter\ in Figure \ref{fig:mse}. The errors are consistently lower when our method is used compared to when the original social network is given as input to \cite{barbieri2013cascade}, thus hinting at a promisingly good capability achievable by the proposed method in extracting the real causal relations within the social network.

\begin{figure}[!t]
\centering
\includegraphics[width=.34\textwidth]{fig/mse_lastfm}
\includegraphics[width=.34\textwidth]{fig/mse_twitter}
\vspace{-4mm}
\captionsetup{justification=justified,singlelinecheck=off,font={stretch=0.7}}
\caption{\footnotesize Mean Squared Error for \lastfm\ (upper panel) and \twitter\ (lower panel), for regularizators AIC and BIC.} \label{fig:mse}
\end{figure}

% \begin{figure}[!t]
% \centering
% \includegraphics[width=.35\textwidth]{fig/mse_twitter}
% \vspace{-4mm}
% \captionsetup{justification=justified,singlelinecheck=off,font={stretch=0.7}}
% \caption{\footnotesize Mean Squared Error for Twitter. We considered $4$ different levels of sampling iterations, $100$, $250$, $500$ and $1000$ and two regularizators, AIC and BIC.} \label{fig:mse_twitter}
% \end{figure}

